Mind2Web: Towards a Generalist Agent for the Web

We introduce Mind2Web, the first dataset for developing and evaluating generalist agents for the web that can follow language instructions to complete complex tasks on any website. Existing datasets for web agents either use simulated websites or only cover a limited set of websites and tasks, thus not suitable for generalist web agents. With over 2,000 open-ended tasks collected from 137 websites spanning 31 domains and crowdsourced action sequences for the tasks, Mind2Web provides three necessary ingredients for building generalist web agents: 1) diverse domains, websites, and tasks, 2) use of real-world websites instead of simulated and simplified ones, and 3) a broad spectrum of user interaction patterns. Based on Mind2Web, we conduct an initial exploration of using large language models (LLMs) for building generalist web agents. While the raw HTML of real-world websites are often too large to be fed to LLMs, we show that first filtering it with a small LM significantly improves the effectiveness and efficiency of LLMs. Our solution demonstrates a decent level of performance, even on websites or entire domains the model has never seen before, but there is still a substantial room to improve towards truly generalizable agents. We open-source our dataset, model implementation, and trained models (https://osu-nlp-group.github.io/Mind2Web) to facilitate further research on building a generalist agent for the web.

==> app_sections/datasheet.tex <==
\newpage
\section{Datasheet}
# Datasheet: *Your Dataset Name Here*

Author: *Your Name Here*

Organization: *Your Organization Here*


## Motivation

*The questions in this section are primarily intended to encourage dataset creators to clearly articulate their reasons for creating the dataset and to promote transparency about funding interests.*

1. **For what purpose was the dataset created?** Was there a specific task in mind? Was there a specific gap that needed to be filled? Please provide a description.

	*Your Answer Here*

2. **Who created this dataset (e.g. which team, research group) and on behalf of which entity (e.g. company, institution, organization)**?

	*Your Answer Here*

3. **What support was needed to make this dataset?** (e.g. who funded the creation of the dataset? If there is an associated grant, provide the name of the grantor and the grant name and number, or if it was supported by a company or government agency, give those details.)

	*Your Answer Here*

4. **Any other comments?**

	*Your Answer Here*


## Composition

*Dataset creators should read through the questions in this section prior to any data collection and then provide answers once collection is complete. Most of these questions are intended to provide dataset consumers with the information they need to make informed decisions about using the dataset for specific tasks. The answers to some of these questions reveal information about compliance with the EU’s General Data Protection Regulation (GDPR) or comparable regulations in other jurisdictions.*

1. **What do the instances that comprise the dataset represent (e.g. documents, photos, people, countries)?** Are there multiple types of instances (e.g. movies, users, and ratings; people and interactions between them; nodes and edges)? Please provide a description.

	*Your Answer Here*

2. **How many instances are there in total (of each type, if appropriate)?**

	*Your Answer Here*

3. **Does the dataset contain all possible instances or is it a sample (not necessarily random) of instances from a larger set?** If the dataset is a sample, then what is the larger set? Is the sample representative of the larger set (e.g. geographic coverage)? If so, please describe how this representativeness was validated/verified. If it is not representative of the larger set, please describe why not (e.g. to cover a more diverse range of instances, because instances were withheld or unavailable).

	*Your Answer Here*

4. **What data does each instance consist of?** "Raw" data (e.g. unprocessed text or images) or features? In either case, please provide a description.

	*Your Answer Here*

5. **Is there a label or target associated with each instance?** If so, please provide a description.

	*Your Answer Here*

6. **Is any information missing from individual instances?** If so, please provide a description, explaining why this information is missing (e.g. because it was unavailable). This does not include intentionally removed information, but might include, e.g. redacted text.

	*Your Answer Here*

7. **Are relationships between individual instances made explicit (e.g. users' movie ratings, social network links)?** If so, please describe how these relationships are made explicit.

	*Your Answer Here*

8. **Are there recommended data splits (e.g. training, development/validation, testing)?** If so, please provide a description of these splits, explaining the rationale behind them.

	*Your Answer Here*

9. **Are there any errors, sources of noise, or redundancies in the dataset?** If so, please provide a description.

	*Your Answer Here*

10. **Is the dataset self-contained, or does it link to or otherwise rely on external resources (e.g. websites, tweets, other datasets)?** If it links to or relies on external resources, a) are there guarantees that they will exist, and remain constant, over time; b) are there official archival versions of the complete dataset (i.e., including the external resources as they existed at the time the dataset was created); c) are there any restrictions (e.g. licenses, fees) associated with any of the external resources that might apply to a future user? Please provide descriptions of all external resources and any restrictions associated with them, as well as links or other access points, as appropriate.

	*Your Answer Here*

11. **Does the dataset contain data that might be considered confidential (e.g. data that is protected by legal privilege or by doctor-patient confidentiality, data that includes the content of individuals' non-public communications)?** If so, please provide a description.

	*Your Answer Here*

12. **Does the dataset contain data that, if viewed directly, might be offensive, insulting, threatening, or might otherwise cause anxiety?** If so, please describe why.

	*Your Answer Here*

13. **Does the dataset relate to people?** If not, you may skip the remaining questions in this section.

	*Your Answer Here*

14. **Does the dataset identify any subpopulations (e.g. by age, gender)?** If so, please describe how these subpopulations are identified and provide a description of their respective distributions within the dataset.

	*Your Answer Here*

15. **Is it possible to identify individuals (i.e., one or more natural persons), either directly or indirectly (i.e., in combination with other data) from the dataset?** If so, please describe how.

	*Your Answer Here*

16. **Does the dataset contain data that might be considered sensitive in any way (e.g. data that reveals racial or ethnic origins, sexual orientations, religious beliefs, political opinions or union memberships, or locations; financial or health data; biometric or genetic data; forms of government identification, such as social security numbers; criminal history)?** If so, please provide a description.

	*Your Answer Here*

17. **Any other comments?**

	*Your Answer Here*


## Collection

*As with the previous section, dataset creators should read through these questions prior to any data collection to flag potential issues and then provide answers once collection is complete. In addition to the goals of the prior section, the answers to questions here may provide information that allow others to reconstruct the dataset without access to it.*

1. **How was the data associated with each instance acquired?** Was the data directly observable (e.g. raw text, movie ratings), reported by subjects (e.g. survey responses), or indirectly inferred/derived from other data (e.g. part-of-speech tags, model-based guesses for age or language)? If data was reported by subjects or indirectly inferred/derived from other data, was the data validated/verified? If so, please describe how.

	*Your Answer Here*

2. **What mechanisms or procedures were used to collect the data (e.g. hardware apparatus or sensor, manual human curation, software program, software API)?** How were these mechanisms or procedures validated?

	*Your Answer Here*

3. **If the dataset is a sample from a larger set, what was the sampling strategy (e.g. deterministic, probabilistic with specific sampling probabilities)?**

	*Your Answer Here*

4. **Who was involved in the data collection process (e.g. students, crowdworkers, contractors) and how were they compensated (e.g. how much were crowdworkers paid)?**

	*Your Answer Here*

5. **Over what timeframe was the data collected?** Does this timeframe match the creation timeframe of the data associated with the instances (e.g. recent crawl of old news articles)? If not, please describe the timeframe in which the data associated with the instances was created. Finally, list when the dataset was first published.

	*Your Answer Here*

7. **Were any ethical review processes conducted (e.g. by an institutional review board)?** If so, please provide a description of these review processes, including the outcomes, as well as a link or other access point to any supporting documentation.

	*Your Answer Here*

8. **Does the dataset relate to people?** If not, you may skip the remainder of the questions in this section.

	*Your Answer Here*

9. **Did you collect the data from the individuals in question directly, or obtain it via third parties or other sources (e.g. websites)?**

	*Your Answer Here*

10. **Were the individuals in question notified about the data collection?** If so, please describe (or show with screenshots or other information) how notice was provided, and provide a link or other access point to, or otherwise reproduce, the exact language of the notification itself.

	*Your Answer Here*

11. **Did the individuals in question consent to the collection and use of their data?** If so, please describe (or show with screenshots or other information) how consent was requested and provided, and provide a link or other access point to, or otherwise reproduce, the exact language to which the individuals consented.

	*Your Answer Here*

12. **If consent was obtained, were the consenting individuals provided with a mechanism to revoke their consent in the future or for certain uses?** If so, please provide a description, as well as a link or other access point to the mechanism (if appropriate).

	*Your Answer Here*

13. **Has an analysis of the potential impact of the dataset and its use on data subjects (e.g. a data protection impact analysis) been conducted?** If so, please provide a description of this analysis, including the outcomes, as well as a link or other access point to any supporting documentation.

	*Your Answer Here*

14. **Any other comments?**

	*Your Answer Here*


## Preprocessing / Cleaning / Labeling

*Dataset creators should read through these questions prior to any pre-processing, cleaning, or labeling and then provide answers once these tasks are complete. The questions in this section are intended to provide dataset consumers with the information they need to determine whether the “raw” data has been processed in ways that are compatible with their chosen tasks. For example, text that has been converted into a “bag-of-words” is not suitable for tasks involving word order.*

1. **Was any preprocessing/cleaning/labeling of the data done (e.g. discretization or bucketing, tokenization, part-of-speech tagging, SIFT feature extraction, removal of instances, processing of missing values)?** If so, please provide a description. If not, you may skip the remainder of the questions in this section.

	*Your Answer Here*

2. **Was the "raw" data saved in addition to the preprocessed/cleaned/labeled data (e.g. to support unanticipated future uses)?** If so, please provide a link or other access point to the "raw" data.

	*Your Answer Here*

3. **Is the software used to preprocess/clean/label the instances available?** If so, please provide a link or other access point.

	*Your Answer Here*

4. **Any other comments?**

	*Your Answer Here*


## Uses

*These questions are intended to encourage dataset creators to reflect on the tasks  for  which  the  dataset  should  and  should  not  be  used.  By  explicitly highlighting these tasks, dataset creators can help dataset consumers to make informed decisions, thereby avoiding potential risks or harms.*

1. **Has the dataset been used for any tasks already?** If so, please provide a description.

	*Your Answer Here*

2. **Is there a repository that links to any or all papers or systems that use the dataset?** If so, please provide a link or other access point.

	*Your Answer Here*

3. **What (other) tasks could the dataset be used for?**

	*Your Answer Here*

4. **Is there anything about the composition of the dataset or the way it was collected and preprocessed/cleaned/labeled that might impact future uses?** For example, is there anything that a future user might need to know to avoid uses that could result in unfair treatment of individuals or groups (e.g. stereotyping, quality of service issues) or other undesirable harms (e.g. financial harms, legal risks) If so, please provide a description. Is there anything a future user could do to mitigate these undesirable harms?

	*Your Answer Here*

5. **Are there tasks for which the dataset should not be used?** If so, please provide a description.

	*Your Answer Here*

6. **Any other comments?**

	*Your Answer Here*


## Distribution

*Dataset creators should provide answers to these questions prior to distributing the dataset either internally within the entity on behalf of which the dataset was created or externally to third parties.*

1. **Will the dataset be distributed to third parties outside of the entity (e.g. company, institution, organization) on behalf of which the dataset was created?** If so, please provide a description.

	*Your Answer Here*

2. **How will the dataset will be distributed (e.g. tarball on website, API, GitHub)?** Does the dataset have a digital object identifier (DOI)?

	*Your Answer Here*

3. **When will the dataset be distributed?**

	*Your Answer Here*

4. **Will the dataset be distributed under a copyright or other intellectual property (IP) license, and/or under applicable terms of use (ToU)?** If so, please describe this license and/or ToU, and provide a link or other access point to, or otherwise reproduce, any relevant licensing terms or ToU, as well as any fees associated with these restrictions.

	*Your Answer Here*

5. **Have any third parties imposed IP-based or other restrictions on the data associated with the instances?** If so, please describe these restrictions, and provide a link or other access point to, or otherwise reproduce, any relevant licensing terms, as well as any fees associated with these restrictions.

	*Your Answer Here*

6. **Do any export controls or other regulatory restrictions apply to the dataset or to individual instances?** If so, please describe these restrictions, and provide a link or other access point to, or otherwise reproduce, any supporting documentation.

	*Your Answer Here*

7. **Any other comments?**

	*Your Answer Here*


## Maintenance

*As with the previous section, dataset creators should provide answers to these questions prior to distributing the dataset. These questions are intended to encourage dataset creators to plan for dataset maintenance and communicate this plan with dataset consumers.*

1. **Who is supporting/hosting/maintaining the dataset?**

	*Your Answer Here*

2. **How can the owner/curator/manager of the dataset be contacted (e.g. email address)?**

	*Your Answer Here*

3. **Is there an erratum?** If so, please provide a link or other access point.

	*Your Answer Here*

4. **Will the dataset be updated (e.g. to correct labeling errors, add new instances, delete instances)?** If so, please describe how often, by whom, and how updates will be communicated to users (e.g. mailing list, GitHub)?

	*Your Answer Here*

5. **If the dataset relates to people, are there applicable limits on the retention of the data associated with the instances (e.g. were individuals in question told that their data would be retained for a fixed period of time and then deleted)?** If so, please describe these limits and explain how they will be enforced.

	*Your Answer Here*

6. **Will older versions of the dataset continue to be supported/hosted/maintained?** If so, please describe how. If not, please describe how its obsolescence will be communicated to users.

	*Your Answer Here*

7. **If others want to extend/augment/build on/contribute to the dataset, is there a mechanism for them to do so?** If so, please provide a description. Will these contributions be validated/verified? If so, please describe how. If not, why not? Is there a process for communicating/distributing these contributions to other users? If so, please provide a description.

	*Your Answer Here*

8. **Any other comments?**

	*Your Answer Here*

==> sections/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See limitations and discussion in Appendix.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See limitations and discussion in Appendix.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See the project website \url{https://osu-nlp-group.github.io/Mind2Web/}.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Section~\ref{sec:data_split}, ~\ref{sec:evaluation} and implementation details in Appendix.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We conducted only one run for the main experiments. The LLM experiments are run with temperature 0. For the few-shot experiments included in Appendix, we repeat the experiments three times with different random sub-samples of the training set and included the error bars.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See implementation details in Appendix.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{See implementation details in Appendix and the project website \url{https://osu-nlp-group.github.io/Mind2Web/}.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{See data collection details in Appendix.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{See data collection details in Appendix.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes{See data collection details in Appendix and the instruction materials provided to the participants in supplementary material.}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerYes{See data collection details in Appendix.}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerYes{See data collection details in Appendix.}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> tables/candidate_pruning.tex <==
\centering
\caption{Candidate generation results.}
\resizebox{\textwidth}{!}{
% \setlength\tabcolsep{3pt}
\begin{tabular}{lcccccc}
\toprule
     & \multicolumn{2}{c}{Cross-Task} & \multicolumn{2}{c}{Cross-Website} & \multicolumn{2}{c}{Cross-Domain}\\
     \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
     &MRR&R@50&MRR&R@50&MRR&R@50\\
     \midrule
    DeBERTa\textsubscript{XS} & 31.6&86.2&25.3&81.8&25.9&80.2\\
    DeBERTa\textsubscript{S} & 34.1&87.5&30.7&79.9&28.8&82.4\\
    DeBERTa\textsubscript{B} & 40.5&88.9&34.6&85.3&35.8&85.7\\
\bottomrule
\end{tabular}}
\label{tab:candidate_prune}

==> tables/data_split.tex <==

\centering
\caption{Data split statistics.}
\resizebox{\textwidth}{!}{
\begin{tabular}{lccc}
\toprule
     &  \# Websites &\# Tasks & \# Steps\\
\midrule
  Train   & \num{73} &\num{1009} &\num{7775}\\
  Test\textsubscript{Cross-Domain} & \num{54} & \num{912} & \num{5911}\\
  Test\textsubscript{Cross-Website} & \num{10} & \num{177} & \num{1373}\\
  Test\textsubscript{Cross-Task} & \num{69} & \num{252} & \num{2094}\\
\bottomrule
\end{tabular}}
\label{tab:data_split}

